Ecologically Valid Explanations for Label Variation in NLI

Human label variation, or annotation disagreement, exists in many natural language processing (NLP) tasks, including natural language inference (NLI). To gain direct evidence of how NLI label variation arises, we build LiveNLI, an English dataset of 1,415 ecologically valid explanations (annotators explain the NLI labels they chose) for 122 MNLI items (at least 10 explanations per item). The LiveNLI explanations confirm that people can systematically vary on their interpretation and highlight within-label variation: annotators sometimes choose the same label for different reasons. This suggests that explanations are crucial for navigating label interpretations in general. We few-shot prompt large language models to generate explanations but the results are inconsistent: they sometimes produces valid and informative explanations, but it also generates implausible ones that do not support the label, highlighting directions for improvement.

==> multilabel_cms.tex <==
\begin{minipage}[h]{.32\textwidth}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
pred & E & N & C & EN & EC & NC & ENC \\
gold &  &  &  &  &  &  &  \\
E & {\cellcolor[HTML]{65AAD4}} \color[HTML]{F1F1F1} 16 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 18 \\
N &   &   & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 &   &   & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 & {\cellcolor[HTML]{1C6AB0}} \color[HTML]{F1F1F1} 24 \\
C &   &   & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 12 &   &   & {\cellcolor[HTML]{3C8CC3}} \color[HTML]{F1F1F1} 20 & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 \\
EN & {\cellcolor[HTML]{D1E2F3}} \color[HTML]{000000} 6 &   &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{1562A9}} \color[HTML]{F1F1F1} 25 \\
EC & {\cellcolor[HTML]{D1E2F3}} \color[HTML]{000000} 6 &   & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 &   &   & {\cellcolor[HTML]{7FB9DA}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 12 \\
NC & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 &   &   & {\cellcolor[HTML]{5BA3D0}} \color[HTML]{F1F1F1} 17 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 11 \\
ENC & {\cellcolor[HTML]{CBDEF1}} \color[HTML]{000000} 7 &   & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 11 & {\cellcolor[HTML]{65AAD4}} \color[HTML]{F1F1F1} 16 \\
\end{tabular}
}\subcaption{Predict-only }
\end{minipage}
\hfill
\begin{minipage}[h]{.32\textwidth}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
pred & E & N & C & EN & EC & NC & ENC \\
gold &  &  &  &  &  &  &  \\
E & {\cellcolor[HTML]{AFD1E7}} \color[HTML]{000000} 10 &   &   & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 11 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 13 \\
N &   & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{CBDEF1}} \color[HTML]{000000} 7 &   & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 12 \\
C &   &   & {\cellcolor[HTML]{AFD1E7}} \color[HTML]{000000} 10 &   &   & {\cellcolor[HTML]{09529D}} \color[HTML]{F1F1F1} 27 &   \\
EN & {\cellcolor[HTML]{D1E2F3}} \color[HTML]{000000} 6 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 & {\cellcolor[HTML]{65AAD4}} \color[HTML]{F1F1F1} 16 \\
EC & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 &   & {\cellcolor[HTML]{CBDEF1}} \color[HTML]{000000} 7 &   & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{7FB9DA}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 \\
NC &   &   & {\cellcolor[HTML]{B9D6EA}} \color[HTML]{000000} 9 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{3484BF}} \color[HTML]{F1F1F1} 21 & {\cellcolor[HTML]{DDEAF7}} \color[HTML]{000000} 4 \\
ENC & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 & {\cellcolor[HTML]{7FB9DA}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{AFD1E7}} \color[HTML]{000000} 10 \\
\end{tabular}
}\subcaption{Predict-then-Explain}
\end{minipage}
\hfill
\begin{minipage}[h]{.32\textwidth}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
pred & E & N & C & EN & EC & NC & ENC \\
gold &  &  &  &  &  &  &  \\
E & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{5BA3D0}} \color[HTML]{F1F1F1} 17 \\
N &   & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{B9D6EA}} \color[HTML]{000000} 9 & {\cellcolor[HTML]{5BA3D0}} \color[HTML]{F1F1F1} 17 & {\cellcolor[HTML]{CBDEF1}} \color[HTML]{000000} 7 \\
C &   &   & {\cellcolor[HTML]{D1E2F3}} \color[HTML]{000000} 6 &   &   & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} 32 &   \\
EN &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{7FB9DA}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 11 \\
EC &   &   & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 &   & {\cellcolor[HTML]{AFD1E7}} \color[HTML]{000000} 10 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 18 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 8 \\
NC & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{DDEAF7}} \color[HTML]{000000} 4 &   & {\cellcolor[HTML]{EAF3FB}} \color[HTML]{000000} 2 & {\cellcolor[HTML]{0F5AA3}} \color[HTML]{F1F1F1} 26 & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 \\
ENC & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{E4EFF9}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{F1F7FD}} \color[HTML]{000000} 1 & {\cellcolor[HTML]{AFD1E7}} \color[HTML]{000000} 10 & {\cellcolor[HTML]{7FB9DA}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{D7E6F5}} \color[HTML]{000000} 5 \\
\end{tabular}
}\subcaption{Explain-then-Predict}
\end{minipage}

==> table_highlight.tex <==

\begin{table*}
  \centering
  \small
  \begin{tabular}{p{\linewidth}}
    \toprule
    \textbf{Agree on label, not on highlights} \\
    \midrule
    \taxex{ex:wreck} \textbf{P}: \colorbox{yellow!20!white}{There} \colorbox{yellow!20!white}{are} \colorbox{yellow!30!white}{other} \colorbox{yellow!40!white}{reasons} \colorbox{yellow!20!white}{that} \colorbox{yellow!80!white}{wrecks} \colorbox{yellow!80!white}{cause} \colorbox{yellow!70!white}{fan} \colorbox{yellow!70!white}{excitement--e.g.}
    \textbf{H}: \colorbox{yellow!40!white}{A} \colorbox{yellow!70!white}{cause} \colorbox{yellow!50!white}{for} \colorbox{yellow!60!white}{fan} \colorbox{yellow!60!white}{excitement} \colorbox{yellow!50!white}{can} \colorbox{yellow!50!white}{be} \colorbox{yellow!80!white}{wrecks.}
    \hfill [E,N,C]: [1, 0, 0] $\alpha$ = 0.08 \\
    \taxex{ex:tommy} \textbf{P}: \colorbox{yellow!10!white}{He} \colorbox{yellow!80!white}{leaned} \colorbox{yellow!50!white}{over} \colorbox{yellow!40!white}{Tommy,} \colorbox{yellow!30!white}{his} \colorbox{yellow!50!white}{face} \colorbox{yellow!80!white}{purple} \colorbox{yellow!30!white}{with} \colorbox{yellow!80!white}{excitement.}
    \textbf{H}: \colorbox{yellow!0!white}{He} \colorbox{yellow!70!white}{hovered} \colorbox{yellow!40!white}{over} \colorbox{yellow!30!white}{Tommy,} \colorbox{yellow!10!white}{with} \colorbox{yellow!20!white}{a} \colorbox{yellow!60!white}{deep} \colorbox{yellow!70!white}{color} \colorbox{yellow!30!white}{in} \colorbox{yellow!30!white}{his} \colorbox{yellow!30!white}{face} \colorbox{yellow!20!white}{from} \colorbox{yellow!20!white}{the} \colorbox{yellow!70!white}{thrill.} \hfill
[E,N,C]: [1, 0, 0] $\alpha$ = 0.15 \\
    \toprule
\textbf{Agree on highlights, not on labels}\\
    \midrule
    \taxex{ex:simile} \textbf{P}: What a brilliantly innocuous \colorbox{yellow!90!white}{metaphor,} \colorbox{yellow!30!white}{devised} \colorbox{yellow!10!white}{by} \colorbox{yellow!10!white}{a} \colorbox{yellow!30!white}{master} \colorbox{yellow!70!white}{manipulator} to obscure his manipulations.
    \textbf{H}: The \colorbox{yellow!90!white}{simile} \colorbox{yellow!10!white}{was} \colorbox{yellow!40!white}{created} \colorbox{yellow!20!white}{by} \colorbox{yellow!30!white}{the} \colorbox{yellow!60!white}{manipulator.}\hspace*{2.27259cm}
    [E,N,C]: [0.3, 0.4, 0.3] $\alpha$ = 0.43 \\
    \Entailment -- As all metaphors are a subset of similes, the statement must be true.\\
    \Neutral -- A metaphor is not the same as a simile, which the manipulator definitely created, but they could have created a simile too.\\
    \Contradiction -- The context describes a metaphor, while the statement mentions a simile, which is a different type of speech.\\
    \bottomrule
  \end{tabular}
  \caption{Examples where agreement on either the label or the
    highlights does not imply agreement on the other. Color transparency indicates the percentage of annotators who highlighted the word.
    The agreement on highlights do not correlate with agreement on labels.
  }
  \label{tab:highlight}
\end{table*}

==> table_taxonomy_reannot.tex <==


\begin{table}[t]
  \footnotesize
  \centering
    \begin{tabulary}{1.0\linewidth}{@{}lr@{}}
\toprule
Combination of Taxonomy Categories &  Frequency \\
\midrule
Probabilistic                &         28 \\
Lexical                      &         21 \\
\textit{QUD}                          &         15 \\
Coreference                  &          6 \\
Lexical | Probabilistic      &          5 \\
Coreference | Probabilistic  &          5 \\
Imperfection | Lexical       &          5 \\
Implicature                  &          5 \\
Imperfection | Probabilistic &          4 \\
Probabilistic | \textit{QUD}          &          4 \\
Coreference | Lexical        &          3 \\
Lexical | \textit{QUD}                &          3 \\
Temporal                     &          2 \\
\midrule
Appear once:\\
\multicolumn{2}{@{}p{\linewidth}@{}}{
Implicature | Interrogative; Implicature | Lexical; Interrogative; Implicature |
\textit{QUD}; Imperfection | \textit{QUD}; Interrogative | Lexical; Coreference | Temporal;
Coreference | Imperfection; Coreference | \textit{QUD};
Implicature | Interrogative; Implicature | Lexical; Interrogative; Implicature |
Lexical | Probabilistic | \textit{QUD}; Probabilistic | Temporal; Presupposition | \textit{QUD}; \textit{QUD} | Temporal
}\\
\bottomrule
\end{tabulary}
  \caption{Frequency of the taxonomy categories in \livenli. Label variation in annotators arises for similar reasons as what \citet{qp2} hypothesized. QUD is a new category.
  }
  \label{tab:taxonomy_reannot}
\end{table}


